DetailSemNet: Elevating Signature Verification through Detail-Semantic Integration

Offline signature verification (OSV) is a frequently utilized technology in forensics. This paper proposes a new model, DetailSemNet, for OSV. Unlike previous methods that rely on holistic features for pair comparisons, our approach underscores the significance of fine-grained differences for robust OSV. We propose to match local structures between two signature images, significantly boosting verification accuracy. Furthermore, we observe that without specific architectural modifications, transformer-based backbones might naturally obscure local details, adversely impacting OSV performance. To address this, we introduce a Detail Semantics Integrator, leveraging feature disentanglement and re-entanglement. This integrator is specifically designed to enhance intricate details while simultaneously expanding discriminative semantics, thereby augmenting the efficacy of local structural matching. We evaluate our method against leading benchmarks in offline signature verification. Our model consistently outperforms recent methods, achieving state-of-the-art results with clear margins. The emphasis on local structure matching not only improves performance but also enhances the model's interpretability, supporting our findings. Additionally, our model demonstrates remarkable generalization capabilities in cross-dataset testing scenarios. The combination of generalizability and interpretability significantly bolsters the potential of DetailSemNet for real-world applications.

==> sec/table_exp.tex <==
% BHSig-H (single)-------------------------------------------------------------------------
\begin{table}[t]
  \caption{Signature verification comparison on BHSig-H(\%) and BHSig-B(\%).}
  \centering
  \begin{tabular}{l||rrrr|rrrr}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c|}{BHSig-H} & \multicolumn{4}{c}{BHSig-B} \\
     & ~FAR & ~FRR & ~Acc $\uparrow$ & ~EER $\downarrow$ & ~FAR & ~FRR & ~Acc $\uparrow$ & ~EER $\downarrow$ \\
    \midrule
    SigNet\cite{dey2017signet}    & 15.36 & 15.36 & 84.64 & 15.36 & 13.89 & 13.89 & 86.11 & 13.89 \\
    IDN\cite{wei:19IDN}           &  4.93 &  8.99 & 93.04 &  6.96 &  4.12 &  5.24 & 95.32 &  4.68 \\
    DeepHsv\cite{Li:19DeepHSV}    &     - &     - & 86.66 & 13.34 &     - &     - & 88.08 & 11.92 \\
    SDINet\cite{Li:21SDINet}      &  6.24 &  3.77 & 95.00 &  5.11 &  3.30 &  7.86 & 94.42 & 5.39 \\
    CaC\cite{Lu:21Cac}            &  5.97 &  5.97 & 94.03 &  5.97 &  3.96 &  3.96 & 96.04 & 3.96 \\
    AVN\cite{Li:22AVN}            &  5.46 &  5.91 & 94.32 &  5.65 &  7.33 &  5.07 & 93.80 & 6.14 \\
    TransOSV\cite{Li02:22TranOSV, TransOSV_PR} &  3.39 &  \textbf{3.39} & 96.61 &  3.39 &  9.95 &  9.95 & 90.05 & 9.95 \\
    % FC-ResNet\cite{FCResNet}      &  3.13 &  2.31 & 97.28 &     - \\
    2C2S\cite{REN2023105639}      &  8.66 &  5.16 & 90.68 &  9.32 &  5.37 &  8.11 & 93.25 & 6.75  \\
    SURDS\cite{SURDS}             & 12.01 &  8.98 & 89.50 &     - & 19.89 &  5.42 & 87.34 &    -  \\
    % SWIS\cite{SWIS}               & 10.40 & 59.80 & 72.43 &     - & 36.70 & 11.60 & 72.04 &    -  \\
    MA-SCN\cite{Zhang2022MASCN}   &  5.73 &  4.86 & 94.99 &  5.32 &  9.96 &  5.85 & 92.86 & 8.18 \\
    SigGCN\cite{Ren2023VisionGC}  & 12.96 & 11.27 & 87.88 & 12.17 &  4.06 &  \textbf{3.95} & 95.99 & 4.00 \\
 Co-Tuplet\cite{Huang2023MultiscaleFL} & 6.76 & 6.56 & - & 6.68 & 5.93 & 6.20 & - & 6.12 \\
 HybridFE\cite{Xiong2023HybridFE} & 11.74 & 11.74 & 88.26 & 11.74 & 8.36  & 8.36  & 91.64 & 8.36 \\
    SPD Manifold\cite{Zois}       &     - &     - &     - & 15.60 &     - &     - &     - & 11.10 \\
    \textbf{Ours}                 &  \textbf{1.07} &  3.59 & \textbf{98.24} &  \textbf{2.07} &  \textbf{0.95} &  4.04 & \textbf{98.19} & \textbf{2.11} \\
    \bottomrule
  \end{tabular}
  % \label{tab:table_BHSig_H}
  \label{tab:table_BHSig_B_H}
\end{table}

% CEDAR (single)-------------------------------------------------------------------------
\begin{table}%[t]
%\begin{wraptable}{r}{0.6\linewidth}
\caption{Signature verification comparison on CEDAR(\%).}
  \centering
  \begin{tabular}{l||rrrr}
    \toprule
    Method & ~FAR & ~FRR & ~Acc $\uparrow$ & ~EER $\downarrow$ \\
    \midrule
    SigNet\cite{dey2017signet} & -    & -    & -     & 4.63 \\
    IDN\cite{wei:19IDN}        & 5.87 & 2.17 & -     & 3.62 \\
    SDINet\cite{Li:21SDINet}   & 3.42 & 0.73 & -     & 1.75 \\
    CaC\cite{Lu:21Cac}         & 4.34 & 4.34 & 95.66 & 4.43 \\
    AVN\cite{Li:22AVN}         & 3.26 & 4.42 & 96.16 & 3.77 \\
 MA-SCN\cite{Zhang2022MASCN}   & 19.21 & 18.35 & 80.75 & 18.92 \\
    MLDF\cite{Arab}            &    - &    - &     - & 5.00 \\
 Co-Tuplet\cite{Huang2023MultiscaleFL} & 3.33 & 3.55 & - & 3.51 \\
 HybridFE\cite{Xiong2023HybridFE} & 9.95 & 9.95 & 90.05 & 9.95 \\
    SPD Manifold\cite{Zois}    &    - &    - &     - & 8.53 \\
    \textbf{Ours}              & \textbf{0.36} & \textbf{0.58} & \textbf{99.53} & \textbf{0.58} \\
    \bottomrule
  \end{tabular}
  \label{tab:table_CEDAR}
%\end{wraptable}
\end{table}

\iffalse
% Cross-BHSig-B-------------------------------------------------------------------------
\begin{table}[t]
\caption{The zero-shot cross-lingual signature verification task (cross-dataset) testing results.}
  \centering
  \begin{subtable}[t]{\columnwidth}
  \caption{Train on BHSig-B dataset. Test on others' EER (\%).}
  \centering
  \begin{tabular}{l||rrrr}
    \toprule
     & \textbf{Ours} & CaC\cite{Lu:21Cac} & IDN\cite{wei:19IDN} & SigNet\cite{dey2017signet} \\
    \midrule
    BHSig-B &  \textbf{2.11} &  3.96 &  4.68 & 13.19 \\
    BHSig-H & \textbf{15.91} & 30.41 & 25.70 & 35.43 \\
    CEDAR   & \textbf{7.32} & 33.71 & 50.00 & 50.00 \\
    \bottomrule
  \end{tabular}
  \label{tab:table_Cross-BHSig-B}
  \end{subtable}

% Cross-BHSig-H-------------------------------------------------------------------------
  \begin{subtable}[h]{\columnwidth}
  \caption{Train on BHSig-H dataset. Test on others' EER (\%).}
  \centering
  \begin{tabular}{l||rrrr}
    \toprule
     & \textbf{Ours} & CaC\cite{Lu:21Cac} & IDN\cite{wei:19IDN} & SigNet\cite{dey2017signet} \\
    \midrule
    BHSig-B & \textbf{7.46} & 14.66 & 25.88 & 39.35 \\
    BHSig-H &  \textbf{2.07} &  5.97 &  6.96 & 15.36 \\
    CEDAR   & \textbf{14.05} & 29.49 & 50.00 & 40.43 \\
    \bottomrule
  \end{tabular}
  \label{tab:table_Cross-BHSig-H}
  \end{subtable}

% Cross-CEDAR-------------------------------------------------------------------------
  \begin{subtable}[h]{\columnwidth}
  \caption{Train on CEDAR dataset. Test on others' EER (\%).}
  \centering
  \begin{tabular}{l||rrrr}
    \toprule
     & \textbf{Ours} & CaC\cite{Lu:21Cac} & IDN\cite{wei:19IDN} & SigNet\cite{dey2017signet} \\
    \midrule
    BHSig-B & \textbf{8.40} & 38.07 & 49.99 & 35.85 \\
    BHSig-H & \textbf{16.35} & 39.08 & 49.64 & 44.39 \\
    CEDAR   &  \textbf{0.58} &  4.34 &  3.62 & 4.63 \\
    \bottomrule
  \end{tabular}
  \label{tab:table_Cross-CEDAR}
  \end{subtable}
  \label{tab:table_Cross}
\end{table}
\fi

\begin{table}[t]
\caption{The zero-shot cross-lingual OSV task (cross-dataset) testing results. (EER\%)} %  on three datasets
\centering
\begin{tabular}{c||rr|rr|rr}
\toprule
Train & \multicolumn{2}{c|}{BHSig-H} & \multicolumn{2}{c|}{BHSig-B} & \multicolumn{2}{c}{CEDAR} \\
\midrule
Test & \multicolumn{1}{c}{~BHSig-B} & \multicolumn{1}{c|}{~CEDAR} & \multicolumn{1}{c}{~BHSig-H} & \multicolumn{1}{c|}{~CEDAR} & \multicolumn{1}{c}{~BHSig-H} & \multicolumn{1}{c}{~BHSig-B} \\ 
\midrule
\multicolumn{1}{l||}{SigNet~\cite{dey2017signet}} & 39.35 & 40.43 & 35.43 & 50.00 & 44.39 & 35.85 \\
\multicolumn{1}{l||}{IDN~\cite{wei:19IDN}} & 25.88 & 50.00 & 25.70 & 50.00 & 49.64 & 49.99 \\
\multicolumn{1}{l||}{CaC~\cite{Lu:21Cac}} & 14.66 & 29.49 & 30.41 & 33.71 & 39.08 & 38.07 \\
\multicolumn{1}{l||}{SURDS~\cite{SURDS}} & 27.74 & - & 32.99 & - & - & - \\
\multicolumn{1}{l||}{TransOSV~\cite{Li02:22TranOSV, TransOSV_PR}} & 18.66 & - & 17.17 & - & - & - \\
\multicolumn{1}{l||}{\textbf{Ours}} & \textbf{7.46} & \textbf{14.05} & \textbf{15.91} & \textbf{7.32} & \textbf{16.35} & \textbf{8.40} \\
\bottomrule
\end{tabular}
\label{tab:table_Cross}
\end{table}

% different architecture on different datasets
\begin{table*}
\caption{Ablation study of Structural Matching (SM), DetailConv Branch (DCB), and SalientConv Branch (SCB). The table presents the results using the abbreviations M, D, and S in that order. Four different datasets are tested.}
\centering
    \begin{tabular}{ccc||rrr|rrr|rrr|rrr}
        \toprule
        \multirow{2}{*}{M} & \multirow{2}{*}{D} & \multirow{2}{*}{S} & \multicolumn{3}{c}{BHSig-H} & \multicolumn{3}{|c}{BHSig-B} & \multicolumn{3}{|c}{CEDAR} & \multicolumn{3}{|c}{ChiSig} \\
        & & & EER & AUC & Acc & EER & AUC & Acc & EER & AUC & Acc & EER & AUC & Acc \\
        \midrule
        $\times$ & $\times$ & $\times$ & 4.70 & 0.991 & 95.82 & 3.37 & 0.995 & 97.14 & 3.41 & 0.994 & 96.81 & 12.47 & 0.947 & 88.68 \\
        \checkmark & $\times$ & $\times$ & 4.67 & 0.992 & 95.88 & 3.29 & 0.995 & 97.22 & 1.99 & 0.998 & 98.08 & 10.69 & 0.964 & 89.82 \\
        $\times$ & \checkmark & $\times$ & 2.72 & 0.997 & 97.70 & 2.51 & 0.997 & 97.44 & 1.45 & 0.999 & 98.77 & 8.91 & 0.972 & 91.73 \\
        $\times$ & $\times$ & \checkmark & 2.87 & 0.997 & 97.69 & 2.66 & 0.997 & 97.68 & 1.59 & 0.998 & 98.41 & 8.65 & 0.977 & 92.62 \\
        $\times$ & \checkmark & \checkmark & 2.62 & 0.997 & 97.80 & 2.50 & 0.997 & 97.89 & 1.74 & 0.999 & 98.59 & 7.00 & \textbf{0.985} & 93.89 \\
        \checkmark & \checkmark & $\times$ & 2.51 & 0.997 & 97.87 & 2.19 & \textbf{0.998} & 98.03 & 1.09 & 0.999 & 98.95 & 8.65 & 0.977 & 91.35 \\
        \checkmark & $\times$ & \checkmark & 2.72 & 0.997 & 97.74 & 2.19 & \textbf{0.998} & 98.15 & 2.10 & 0.998 & 98.19 & 6.36 & 0.983 & 93.89 \\
        \checkmark & \checkmark & \checkmark & \textbf{2.07} & \textbf{0.998} & \textbf{98.24} & \textbf{2.11} & \textbf{0.998} & \textbf{98.19} & \textbf{0.58} & \textbf{1.000} & \textbf{99.53} & \textbf{5.85} & \textbf{0.985} & \textbf{94.40} \\
        \bottomrule
    \end{tabular}
    \label{tab:table_ablation_dataset}
\end{table*}

% ablation different stage-------------------------------------------------------------------------

% Use wraptable
\begin{wraptable}{r}{0.45\linewidth}
%\begin{table}[ht]
%\centering
%\begin{minipage}[t]{0.45\linewidth}
    \centering
    \caption{Apply Structural Matching to different stages on the BHSig-H.}
        \begin{tabular}{l || r}
            \toprule
            & EER(\%) $\downarrow$ \\
            \midrule
            stage 3                  & 3.47          \\
            stage 3 \& 4             & 3.05          \\ 
            \textbf{stage 4 (Ours)}  & \textbf{2.09} \\
            \bottomrule
        \end{tabular}
    \label{tab:ablation_diff_stage}
% Use wraptable
\end{wraptable}
\begin{wraptable}{r}{0.45\linewidth}
%\end{minipage}
%\quad
%\begin{minipage}[t]{0.5\linewidth}
    \centering
    \caption{Comparison of Different Backbones. We test our results on the BHSig-H and BHSig-B. All the models are under identical conditions.}
    %\caption{Comparison of Different Backbones. All the models are under identical conditions.}
        \begin{tabular}{l || r r | r r}
            \toprule
            \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{BHSig-H} & \multicolumn{2}{c}{BHSig-B} \\
             & EER & Acc & ERR & Acc \\
            \midrule
            PVT\cite{PVT} & 4.62 & 96.06 & 2.72 & 97.55 \\
            Swin\cite{Swin} & 4.24 & 96.15 & 10.27 & 91.01 \\
            SPACH\cite{SPACH} & 3.71 & 96.67 & 3.30 & 96.90 \\
            DAT\cite{DAT} & 4.94 & 95.73 & 20.09 & 82.77 \\
            BiFormer\cite{biformer} & 4.38 & 96.10 & 8.66 & 92.38 \\
            \textbf{Ours} &\textbf{2.07} & \textbf{98.24} & \textbf{2.11} & \textbf{98.19}\\
            \bottomrule
        \end{tabular}
    \label{tab:table_different_backbone}
% Use wraptable
\end{wraptable}
%\end{minipage}
%\end{table}


\iffalse
\begin{table}
\caption{Ablation study: Apply Structural Matching to different stages on BHSig-H.}
\centering
\begin{tabular}{l||rr}
\toprule
        & EER(\%) $\downarrow$ & AUC $\uparrow$     \\
\midrule
stage 3                  & 3.47              & 0.9960           \\
stage 3 \& 4             & 3.05              & 0.9957           \\ 
\textbf{stage 4 (Ours)}  & \textbf{2.09}     & \textbf{0.9980}  \\
\bottomrule
\end{tabular}
%\captionof{table}{Ablation study: Apply Structural Matching to different stages on BHSig-H.}
\label{tab:ablation_diff_stage}
\end{table}

% different backbone ---------------------------------------------------------
\begin{table}
\caption{Comparison of Different Backbones. We test our results on the BHSig-H and the BHSig-B. All the models are under identical conditions.}
    \centering
    \begin{tabular}{l||rrr|rrr}
        \toprule
        \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{BHSig-H} & \multicolumn{3}{c}{BHSig-B} \\
         & EER & AUC & Acc & ERR & AUC & Acc \\
        \midrule
        PVT\cite{PVT} & 4.62 & 0.991 & 96.06 & 2.72 & 0.996 & 97.55 \\
        Swin\cite{Swin} & 4.24 & 0.993 & 96.15 & 10.27 & 0.967 & 91.01 \\
        SPACH\cite{SPACH} & 3.71 & 0.994 & 96.67 & 3.30 & 0.994 & 96.90 \\
        DAT\cite{DAT} & 4.94 & 0.990 & 95.73 & 20.09 & 0.885 & 82.77 \\
        BiFormer\cite{biformer} & 4.38 & 0.991 & 96.10 & 10.27 & 0.967 & 91.01 \\
        Ours &\textbf{2.07} & \textbf{0.998} & \textbf{98.24} & \textbf{2.11} & \textbf{0.998} & \textbf{98.19}\\
        \bottomrule
    \end{tabular}
%\captionof{table}{Comparison of Different Backbones. We test our results on the BHSig-H and the BHSig-B. All the models are under identical conditions.}
\label{tab:table_different_backbone}
\end{table}
\fi

==> table/ablation_backbone.tex <==
\begin{wraptable}{r}{0.5\linewidth}
    \centering
    \caption{Comparison of Different Backbones. We test our results on the BHSig-H and BHSig-B. All the models are under identical conditions.}
        \begin{tabular}{l || r r | r r}
            \toprule
            \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{BHSig-H} & \multicolumn{2}{c}{BHSig-B} \\
             & EER & Acc & ERR & Acc \\
            \midrule
            PVT\cite{PVT} & 4.62 & 96.06 & 2.72 & 97.55 \\
            Swin\cite{Swin} & 4.24 & 96.15 & 10.27 & 91.01 \\
            SPACH\cite{SPACH} & 3.71 & 96.67 & 3.30 & 96.90 \\
            DAT\cite{DAT} & 4.94 & 95.73 & 20.09 & 82.77 \\
            BiFormer\cite{biformer} & 4.38 & 96.10 & 8.66 & 92.38 \\
            \textbf{Ours} &\textbf{2.07} & \textbf{98.24} & \textbf{2.11} & \textbf{98.19}\\
            \bottomrule
        \end{tabular}
    \label{tab:table_different_backbone}
% Use wraptable
\end{wraptable}

==> table/ablation_stage.tex <==
% ablation different stage-------------------------------------------------------------------------

% Use wraptable
\begin{wraptable}{l}{0.35\linewidth}
    \centering
    \caption{Apply Structural Matching to different stages on the BHSig-H.}
        \begin{tabular}{l || r}
            \toprule
            stage & EER(\%) $\downarrow$ \\
            \midrule
            3                  & 3.47          \\
            3 \& 4             & 3.05          \\ 
            \textbf{4 (Ours)}  & \textbf{2.09} \\
            \bottomrule
        \end{tabular}
    \label{tab:ablation_diff_stage}
% Use wraptable
\end{wraptable}

